A shape variation result via the geometry of eigenfunctions

We discuss some of the geometric properties, such as the foliated Schwarz symmetry, the monotonicity along the axial and the affine-radial directions, of the first eigenfunctions of the Zaremba problem for the Laplace operator on annular domains. These fine geometric properties, together with the shape calculus, help us to prove that the first eigenvalue is strictly decreasing as the inner ball moves towards the boundary of the outer ball.

==> shape1.tex <==
%\newpage
\section{Shape calculus}\label{Shape}
%
In this section, we derive the shape derivative formula for the first eigenvalue of the Laplace operator with the mixed boundary conditions on a bounded domain. First, we recall the concept of a shape (domain) functional on an admissible family of subsets of $\RN$, and we study its variations under certain domain perturbations.
%
\begin{definition}[Shape functional]
	Let $\emptyset \neq D\subseteq \RN$ be an open set and let $\P(D)$ be the power set of $D$. A shape functional $J$ is a map from an admissible family $\A \subseteq \P(D)$ into $\R$.
\end{definition}
%
To study the variations of a shape functional $J$ at a domain $\Om \in \A$, first we consider a family of perturbations of $\Om \subset \RN$ given as follows: 
%by a transformation $\Phi _\eps :\RN \longrightarrow \RN $ of the following form:
%
\begin{equation}\label{trans}
    \left.
	\begin{array}{c}
	\text{for a fixed vector field } V\in W^{3,\infty }(\RN ,\RN) \text{ we consider the transformations}\\ \Phi _\eps (x)=(I+\eps V)x=x+\eps V(x) \quad \mbox{for } x\in \RN ,\ \eps \in [0,\eps _0) \mbox{ for some small } \eps _0 >0;
	\end{array}
	\right\}
\end{equation}
%\begin{equation}\label{trans}
%	\text{for a fixed vector field } V\in W^{k,\infty }(\RN ,\RN) \text{ with } k\geq 3, \Phi _\eps (x)=(I+\eps V)x=x+\eps V(x) \quad \mbox{ for } x\in \RN ,\ \eps \in [0,\eps _0 )\mbox{ for some small } \eps _0 >0.
%\end{equation}
%
%where $V\in W^{k,\infty }(\RN ,\RN)$ is a fixed vector field with $k\geq 3$. %and we use the concept of Eulerian derivative of the shape functionals. 
and a family of perturbed domains
%, for a fixed vector field $V\in W^{k,\infty }(\RN ,\RN) \text{ with } k\geq 3,$ is 
%given by 
\begin{equation}\label{admisfamily}
\A \dq \Big\{\Om _\eps =\Phi _\eps (\Om ): \eps \in [0,\eps _0 )\Big\}\text{
	for some small }\eps _0 >0.
\end{equation}
%
\begin{definition}[Eulerian derivative]\label{Def:shape}
	Let	$V$ be a vector field as given in~\eqref{trans}, and $J$ be a shape functional. The Eulerian derivative of the shape functional $J$ at $\Om \in \A$ in the direction of $V$ is defined as the following limit, if it exists:
	
	\noindent
	\begin{equation*}
		dJ(\Om ;V)=\lim\limits_{\eps \searrow 0} \frac{J(\Om _\eps ) -J(\Om )}{\eps },
	\end{equation*}
	where $\Om _\eps =\Phi_\eps (\Om )\mbox{ and }\Phi _\eps$ is given by~\eqref{trans}.
\end{definition}
%
%Some examples of shape functionals are as follows:
%\[J_1(\Om )=|\Om |=\int _\Om \dx,\, J_2(\Om )=|\pa \Om | =\int _{\pa \Om }\dS,\]
%\[J_3(\Om )=\int _\Om C(u)\dx \mbox{ for a differential operator } C.\]
%From the definition, we have
%\[dJ_1(\Om ;V)=\int _\Om \mbox{div}(V)\dx=\int _{\pa \Om }(V\cdot n) \dS;\]
%%
%\begin{equation}\label{shape derivative}
%    dJ_3(\Om ;V)=\int _\Om \frac{\pa C}{\pa u}u'\dx +\int _{\pa \Om }C(u)(V\cdot n)\dS,
%\end{equation}
%%
%where $u'$ %$u'=\left.\frac{\pa}{\pa t}u(t,x)\right|_{t=0}$ 
%is the shape derivative of $u$ in the direction of $V$. 
In many of the physical situations, a shape functional $J(\Om )$ depends on the domain via the solution $u(\Om )$ of a boundary value problem defined in $\Om $. We call $u(\Om )$ as the shape function. The Eulerian derivative of such $J(\Om )$ depends on so called the shape derivative of $u(\Om )$. %\tr{Now, we define the material derivative of a shape function $u(\Om )$, which can be obtained by a certain rule on the domain~$\Om $ such as a solution of a boundary value problem on~$\Om $.}
%
\begin{definition}[Material derivative]
	\label{defn:mat_deri}
	Let	$V$ be a vector field as given in~\eqref{trans}. For a shape function $u(\Om )\in W^{1,p}(\Om )$ with $1\leq p <\infty $, the material derivative $\dot{u}=\dot{u}(\Om ;V)$ in the direction of $V$ is defined as the following limit, if it exists:
	
	\noindent
	\begin{equation*}
		\dot{u}(\Om ;V)=\lim \limits _{\eps \searrow 0} \frac{1}{\eps } \Big(u(\Om _\eps )\circ \Phi _\eps - u(\Om ) \Big)\mbox{ in } W^{1,p}(\Om ),
	\end{equation*}
	where
	$\Om _\eps =\Phi _\eps (\Om ) \mbox{ and }\Phi _\eps$ is given by \eqref{trans}.
\end{definition}
%
\begin{definition}[Shape derivative]
	\label{defn:shape_der}
	Let	$V$ be a vector field as given in~\eqref{trans}. For a shape function $u(\Om )\in W^{1,p}(\Om )$, if the material derivative $\dot{u}(\Om ;V)$ exists and $\nabla u(\Om ) \cdot V\in L^p(\Om ),$ then  the shape derivative $u'=u'(\Om ;V)$ in the direction of $V$ is defined as
	\begin{equation}\label{eq:shape}
		u'(\Om ;V)=\dot{u}(\Om ;V)-\nabla u(\Om )\cdot V.
	\end{equation} 
\end{definition}
%
\begin{remark}
	We observe that, for a transformation $\Phi _\eps $ given in \eqref{trans}, for any compact set $K\subset \Om $ there exists $\eps _K>0$ such that $\Phi _\eps (K)\subset \Om $ for $\eps \leq \eps _K$. Therefore, the shape derivative of $u$ can be defined locally on every compact set as the derivative of $\eps \longmapsto \left. u(\Om _\eps )\right |_{K}$ in $K$. The material derivative of $u$ is the derivative of $\eps \longmapsto u(\Om _\eps )\circ \Phi _\eps $ in $\Om $. If the material derivative of $u$ exists then, from \cite[Corollary~5.2.3 or Lemma~5.2.7]{Henrot-Book}, the shape derivative exists and is given by \eqref{eq:shape}.
\end{remark}
%
\subsection{Shape derivative of the eigenfunctions and the eigenvalues}
Let $\Om \subset \RN$ be a bounded domain and let $\pa \Om =\Ga _D\cup \Ga _N$. We consider the following eigenvalue problem on $\Om :$
%Let $u$ be an eigenfunction corresponding to a simple eigenvalue $\tau _1(\Om )$ of the following eigenvalue problem on $\Om $ with $\pa \Om =\Ga _D\cup \Ga _N$:
\begin{equation}\label{eigen1}
\left.
%
\begin{aligned} 
-\De u & = \tau u \mbox{ in } \Om ,\\
u &= 0 \mbox{ on } \Ga _D,\\
\frac{\pa u}{\pa n} &= 0  \mbox{ on } \Ga _N.
\end{aligned}
%
\right\}
\end{equation}
%
Next, we give the existence of the material derivative of the normalize eigenfunction $u(\Om )$ corresponding to the first eigenvalue $\tau _1(\Om )$ of~\eqref{eigen1}. See~\cite[Lemma 3.18, page 154]{Soko}, for the material derivative for a non-homogeneous problem with the mixed boundary conditions. For a vector field $V$ given in~\eqref{trans}, let $\Om _\eps $ be %For given vector field $V\in W^{k,\infty }(\RN ,\RN)$, consider the family of perturbations of the domain $\Om $ 
as given in \eqref{admisfamily} with the boundary $\pa \Om _\eps = \Ga _D^\eps \sqcup \Ga _N^\eps $, where $\Ga _i^\eps =\Phi _\eps (\Ga _i)$ for $i=D,N$. Let $(u_\eps , \tau _1(\eps ))$ be the first eigenpair of~\eqref{eigen1} in $\Om _\eps $ such that $\int _{\Om _\eps }u_\eps ^2\dx =1.$ We adapt the ideas of \cite[Theorem~5.3.2 and Theorem~5.7.2]{Henrot-Book} and show that both the material and the shape derivatives of $u(\Om )$ exist. %mapping $\eps \longmapsto (u_\eps , \tau (\eps ))$ is differentiable at $0$. It is stated in the following proposition.
%
\begin{proposition}\label{mat_der}
	Let $\tau _1(\Om )$ be the first eigenvalue of~\eqref{eigen1} in $\Om $ and let $u(\Om )$ be a corresponding eigenfunction with $\int _{\Om }u(\Om )^2\dx=1.$ Let	$V$ be a vector field as given in~\eqref{trans}. Then, %the maps $\eps \longmapsto (u(\Om _\eps)\circ \Phi _\eps , \tau (\Om _\eps ))$ and $\eps \longmapsto u(\Om _\eps)$ are differentiable at $0$. In other words, 
	both the material derivative and the shape derivative of $u(\Om )$ exist, and also the Eulerian derivative of the shape functional $\tau _1(\Om )$ exists.
\end{proposition}
%
\begin{proof}
	Let $u_\eps \in \hd{\eps }$ be the eigenfunction corresponding to the first eigenvalue $\tau _1(\Om _\eps )$ of~\eqref{eigen1} on $\Om _\eps $ for $\eps \in [0,\eps _0)$ with the normalization $\int_{\Om _\eps }u_\eps ^2\dx=1$ , i.e.,
	%
	
	\noindent
	\begin{equation*}
	%u_\eps \in \hd{\eps }, \int_{\Om _\eps }u_\eps ^2\dx=1: 
	\int _{\Om _\eps } \nabla u_\eps \cdot \nabla \varphi \dx -\tau _1(\Om _\eps ) \int _{\Om _\eps } u_\eps \varphi \dx =0 \quad \forall \varphi \in \hd{\eps }.
	\end{equation*}
	%
	Let $v_\eps $ be $v_\eps =u_\eps \circ \Phi _\eps$ in $\Om $ for $\eps \in [0,\eps _0)$. For $\eps =0,$ we have $\Om _0 =\Om $ and $v_0=u_0=u(\Om )$. We observe that $v_\eps \in \HD{}$ and satisfies
	\begin{equation}\label{eqn:material1}
		\int _{\Om } \big(A(\eps )\nabla v_\eps \big)\cdot \nabla \psi \dx-\tau _1(\Om _\eps ) \int _{\Om }\ga (\eps ) v_\eps \psi \dx =0 \quad \forall \psi =\varphi \circ \Phi _\eps \in \HD{},
	\end{equation}
	%
	where $A(\eps )=\ga (\eps )D\Phi _\eps ^{-1} ({D\Phi _\eps ^{-1}})^T,$ $\ga (\eps ) =\left |\det(D\Phi _\eps )\right | \mbox{ for }\eps \in [0,\eps _0 ).$ Thus, $v_\eps $ satisfies the following equation:
	
	\noindent
	\begin{equation*}
		-\mathrm{div}(A(\eps )\nabla v_\eps )=\tau _1(\Om _\eps )\ga (\eps ) v_\eps \mbox{ in }\Om .
	\end{equation*}
	Now, we consider the %following 
	function $\F :[0,\eps _0)\times \HD{}\times \R \longrightarrow H^{-1}(\Om )\times \R$ defined by
	
	\noindent
	\begin{equation*}
		\F (\eps ,v,\tau )=\left (-\mathrm{div}(A(\eps )\nabla v )-\tau \ga (\eps ) v , \int_{\Om }v^2 \dx -1\right ).
	\end{equation*}
	Then $\F$ is well-defined and continuous. We observe that 
	$\F(\eps ,v_\eps , \tau _1(\Om _\eps ))=(0,0)\ \text{(by~\eqref{eqn:material1})}$ 
	and
	
	\noindent
	\begin{equation*}
		D_{v,\tau _1}\F(0,u(\Om ), \tau _1(\Om ))(\phi ,\tau _1)
		=\left(-\De \phi -\tau _1(\Om )\phi -\tau _1u(\Om ) ,2\int_{\Om }u(\Om ) \phi \dx \right).
	\end{equation*}
	From~\cite[Lemma 5.7.3]{Henrot-Book}, it follows that $D_{v,\tau _1}\F(0,u , \tau _1(\Om ))$ is a bijection from $\HD{} \times \R$ onto $H^{-1}(\Om ) \times \R$. Since $D_{v,\tau _1}\F(0,u , \tau _1(\Om ))$ is a continuous linear map, it %and from \cite[Lemma 5.7.3]{Henrot-Book}, it follows that $D_{v,\tau _1}\F(0,u , \tau _1(\Om ))$ is one-to-one. Therefore, 
	%$D_{v,\tau _1}\F(0,u(\Om ), \tau _1(\Om ))$ 
	is an isomorphism from $\HD{} \times \R$ onto $H^{-1}(\Om ) \times \R$. Thus, by the implicit function theorem, there exists a unique map $\eps \longmapsto (v(\eps ),\tau (\eps ))\in \HD{} \times \R $ of class $\C^1 $ on a neighborhood $\mathcal{U}$ of $0$ %and a neighborhood $\mathcal{V}$ of $(u(\Om ), \tau _1(\Om ))$ 
	into $\HD{} \times \R$ such that
 	
 	\noindent
 	\begin{equation*}
 		v(0)=u(\Om ),\quad \tau (0)=\tau _1(\Omega ), \quad \F(\eps ,v(\eps ),\tau _1(\eps ))=(0,0) \mbox{ for } \eps \in \mathcal{U}. 
 	\end{equation*}
 	By the uniqueness, it follows that $v(\eps )=v_\eps \mbox{ and }\tau (\eps )=\tau _1(\Om _\eps )$ for $\eps \in \mathcal{U}$. Since the map $\eps \longmapsto (v_\eps , \tau _1(\Om _\eps ))$ is differentiable at $\eps =0$, the Eulerian derivative of $\tau _1(\Om )$ and the material derivative of $u(\Om )$ in the direction of $V$ exist. Hence, from \cite[Corollary~5.2.3 or Lemma~5.2.7]{Henrot-Book}, the map $\eps \longmapsto u_\eps$ is differentiable at $\eps =0$, i.e., the shape derivative of $u(\Om )$ in the direction of $V$ exists.
\end{proof}
%
\begin{lemma}
	Let $u\in \HD{} $ be an eigenfunction corresponding to the first eigenvalue $\tau _1(\Om )$ of~\eqref{eigen1} in $\Om $. Let	$V$ be a vector field as given in~\eqref{trans}. Then, the material derivative $\dot{u}=\dot{u}(\Om ;V)$ of the eigenfunction $u$ is in $\HD{}$ and it is the unique solution of the following integral equation 
    \begin{equation}\label{eqn:material}
    	%\dot{u}\in \HD{}: \\ 
    	\int _{\Om } \nabla \dot{u}\cdot \nabla \varphi \dx-\tau _1\int _{\Om } \dot{u} \varphi \dx =\int _{\Om } \big(\tau _1'u+\tau _1u\,\mathrm{div}(V)\big)\varphi \dx -\int _{\Om } (A'(0)\nabla u)\cdot \nabla \varphi \dx \quad %\\
    	\forall \varphi \in \HD{}.%,
    \end{equation}
    %
%    \begin{equation}\label{eqn:material}
%    \dot{u}\in \HD{}: \int _{\Om } \nabla \dot{u}\cdot \nabla \varphi \dx-\tau _1\int _{\Om } \dot{u} \varphi \dx =\int _{\Om }\big(\tau _1'u+\tau _1u{\ \rm div}(V)\big)\varphi \dx -\int _{\Om } (A'(0)\nabla u)\cdot \nabla \varphi \dx\qquad
%    \forall \varphi \in \HD{},
%    \end{equation}
    %
   where $A'(0)=\mathrm{div}(V)I-DV-{DV}^T$, $\tau _1'=d\tau _1(\Om ;V)$ the Eulerian derivative of $\tau _1(\Om )$ in the direction of $V$ at $\Om $.
\end{lemma}
%
\begin{proof}
%	Let $u_\eps \in \hd{\eps }$ be an eigenfunction corresponding to a simple eigenvalue $\tau _1_1(\Om _\eps )$ of~\eqref{eigen1} on $\Om _\eps $ for $\eps \in [0,\eps _0)$, i.e.,
%	
%	\noindent
%	\begin{equation*}
%	    u_\eps \in \hd{\eps }: \int _{\Om _\eps } \nabla u_\eps \cdot \nabla \varphi \dx -\tau _1(\Om _\eps ) \int _{\Om _\eps } u_\eps \varphi \dx =0 \quad \forall \varphi \in \hd{\eps },
%	\end{equation*}
%	%
%	where $\Om _\eps =\Phi _\eps (\Om )$ and $\Ga _D^\eps =\Phi _\eps (\Ga _D)$. Let $u^\eps $ be stand for
%	\[u^\eps =u_\eps \circ \Phi _\eps \in \HD{}.\]
%	Then
%	%
%	\begin{equation}\label{eqn:material1}
%        u^\eps \in \HD{}: \int _{\Om } \big(A(\eps )\nabla u^\eps \big)\cdot \nabla \psi \dx-\tau _1(\Om _\eps ) \int _{\Om }\ga (\eps ) u^\eps \psi \dx =0 \quad \forall \psi =\varphi \circ \Phi _\eps \in \HD{},
%    \end{equation}
%    %
%    where $A(\eps )=\ga (\eps )D\Phi _\eps ^{-1} ({D\Phi _\eps ^{-1}})^T,$ $\ga (\eps )=\left |\det(D\Phi _\eps )\right | \mbox{ for }\eps \in [0,\eps _0 ).$ Since $u_\eps \in \hd{\eps }$, from \cite[Lemma 5.3.3]{Henrot-Book}, we get that
    By Proposition~\ref{mat_der}, the map $\eps \longmapsto u_\eps$ is differentiable, i.e., the material derivative $\dot{u}(\Om ;V)$ exists and is in $\HD{}$. Therefore, by differentiating the equation~\eqref{eqn:material1} with respect to $\eps $ at $\eps =0$, we get that
    
    \noindent
    \begin{equation*}
    	%\dot{u}\in \HD{}:
    	\int _\Om (A'(0)\nabla u)\cdot \nabla \varphi \dx + \int _\Om \nabla \dot{u}\cdot \nabla \varphi \dx - \int _\Om \dot{(\tau _1u)} \varphi \dx -\tau _1\int _\Om u\ga '(0)\varphi \dx =0\quad \forall \varphi \in \HD{},
    \end{equation*}
    %
    with $A'(0)=\mathrm{div}(V)I-DV-{DV}^T$.
    Noting that $\ga '(0)={\rm div}(V)$ and using the product rule for the material derivative, we obtain~\eqref{eqn:material}.
\end{proof}
%
\begin{remark}
	The material derivative of an eigenfunction $u(\Om )\in \HD{}$ corresponding to the first eigenvalue $\tau _1(\Om )$ of~\eqref{eigen1} in $\Om $, is the unique weak solution of the following boundary value problem:
	
	\noi
	\begin{equation*}
		\left.
		\begin{aligned}
		-\De \dot{u}-\tau _1(\Om ) \dot{u}&=f(u)\text{ in } \Om ,\\
		\dot{u} &=0\text{ on }\Ga _D,\\
		\frac{\pa \dot{u}}{\pa n} &= -(A'(0)\nabla u)\cdot n \text{ on } \Ga _N,
		\end{aligned}
		\right\}
	\end{equation*}
	with $f(u)=(\tau _1'+\tau _1\,\mathrm{div}(V))u+\mathrm{div}(A'(0)\nabla u).$
    %
\end{remark}
%

\par From the definition of the shape derivative of $u$, we have the following lemma.
%
\begin{lemma}\label{shape:lemma0}
	Let	$V$ be a vector field as given in~\eqref{trans}. The shape derivative $u'=u'(\Om ;V)$ of the eigenfunction $u(\Om )$ corresponding to the first eigenvalue $\tau _1(\Om )$ of~\eqref{eigen1} in $\Om $, is the unique weak solution of the following boundary value problem:
	
	\noindent
    \begin{equation*}
		\left.
		\begin{aligned}
			-\De u'&=\tau _1(\Om ) u'+ \tau _1' u \text{ in } \Om ,\\
			u' &= -\frac{\pa u}{\pa n}\, (V\cdot n) \text{ on } \Ga _D,\\
			\frac{\pa u'} {\pa n} &= -\big(A'(0)\nabla u+\nabla (\nabla u \cdot V)\big)\cdot n %(DV\nabla u)\cdot n -\nabla ^2 uV\cdot n 
			\text{ on } \Ga _N.
		% ,\\
		% & &\displaystyle 2\int_{\Om}u u^{\prime} + \int_{\Ga_N}u^2\, (V\cdot n) \dS=0.
	    \end{aligned}
	   \right\}
    \end{equation*}
    %
    %where $(\nabla ^2u V)_j=\displaystyle \nabla \left(\frac{\pa u}{\pa x_j}\right)\cdot V.$
\end{lemma}
%
\begin{proof}
	Using the definition of $u'=\dot{u}-\nabla u\cdot V$ in $\Om $, we rewrite \eqref{eqn:material} as
    %\begin{multline}
    % \forall\varphi\in\D(\Om):\\ \int_\Om \nabla u'\cdot\nabla \varphi\dx-\tau\int_\Om u'\varphi\dx-\tau'\int_\Om u\varphi\dx=-\int_\Om \nabla(\nabla u\cdot V)\cdot\nabla\varphi\dx+\tau\int_\Om(\nabla u\cdot V)\varphi\dx\\+\tau\int_\Om u{\ \rm div}(V)\varphi\dx-\int_\Om (A'(0)\nabla u)\cdot \nabla \varphi\dx.
    %\end{multline}
    %
    \begin{equation}\label{eqn:material-1}
    	%\forall \varphi \in \D (\Om ):
    	\int _\Om \nabla u'\cdot \nabla \varphi \dx -\tau _1\int _\Om u'\varphi \dx -\tau _1'\int _\Om u\varphi \dx
    	=-\int _\Om \big( \nabla (\nabla u\cdot V)- (A'(0)\nabla u)\big)\cdot \nabla \varphi \dx +\tau _1\int _\Om \mathrm{div}(uV)\varphi \dx.
    \end{equation}
    %
    %
%    \begin{equation}\label{eqn:material-1}
%    \forall \varphi \in \D (\Om ):
%    \int _\Om \nabla u'\cdot \nabla \varphi \dx -\tau _1\int _\Om u'\varphi \dx -\tau _1'\int _\Om u\varphi \dx\\
%    =-\int _\Om \big( \nabla (\nabla u\cdot V)- (A'(0)\nabla u)\big)\cdot \nabla \varphi \dx +\tau _1\int _\Om {\rm div}(uV)\varphi \dx.
%    \end{equation}
    %
    We claim that
    
    \noindent
    \begin{equation*}\label{shape:eqn1}
        \int _\Om \big(\nabla (\nabla u\cdot V)+ (A'(0)\nabla u) \big) \cdot \nabla \varphi \dx-\tau _1\int _\Om \mathrm{div} (uV)\varphi \dx =0 \quad \forall \varphi \in \D (\Om ).
    \end{equation*}
    For this, we define $f(u,V)\dq A'(0)\nabla u +\nabla (\nabla u \cdot V)-\De u V$ in $\Om $. It is easy to verify that $\mathrm{div}(f(u,V))=0$. %We recall the identity $\nabla (\nabla u\cdot V)=\nabla ^2 u V+{DV}^T\nabla u$.
    Now, for $\varphi \in \D(\Om )$, we have
    %
    \begin{eqnarray*}
    	\int _\Om \big(\nabla (\nabla u\cdot V)\!
    	+\! A'(0)\nabla u\big)\cdot \nabla \varphi \dx%\\
    	%&=& \int _\Om \Big(\nabla ^2uV+DV^T\nabla u+\mathrm{div}(V)\nabla u
    	%-DV\nabla u-DV^T\nabla u\Big)\cdot \nabla \varphi \dx\\
    	&=& \int _\Om \Big(f(u,V)+\De u V\Big)\cdot \nabla \varphi \dx\\
    	&=& -\int _\Om \mathrm{div}(f(u,V))\varphi \dx
    	+\int _{\pa \Om }\varphi f(u,V)\cdot n\dS -\tau _1\int _\Om u V\cdot \nabla \varphi \dx\\
    	&=& -0+0-\tau _1\int _\Om u V\cdot \nabla \varphi \dx\\
    	&=&\tau _1\int _\Om \mathrm{div}(uV)\varphi \dx
    	-\tau _1\int _{\pa \Om }\varphi u V\cdot n \dS
    	=\tau _1\int _\Om \mathrm{div}(uV)\varphi \dx. %\qedhere
    \end{eqnarray*}
    The last equality follows from the integration by parts.
    %
    Therefore, \eqref{eqn:material-1} gives:
    
    \noindent
    \begin{equation*}
    	\int _\Om \nabla u'\cdot \nabla \varphi \dx -\tau _1\int _\Om u'\varphi \dx -\tau _1'\int _\Om u\varphi \dx=0 \quad \forall \varphi \in \D (\Om ).
    \end{equation*}
    Now, using the integration by parts we get
       
    \noindent
    \begin{equation*}
    	-\int _\Om \De u' \varphi \dx - \tau _1\int _\Om u' \varphi \dx -\tau _1' \int _\Om u \varphi \dx=0 \quad \forall \varphi \in \D (\Om ),
    \end{equation*}
    %
%    Therefore,
%    \[\int _\Om (-\De u'-\tau _1u' -\tau _1u)\varphi \dx =0 \quad \forall \varphi \in \D (\Om ),\]
    and hence
    
    
    \noindent
    \begin{equation*}
    	-\De u'=\tau _1u' +\tau _1' u \text{ in }\Om .
    \end{equation*}
    Since $u=0$ on $\Ga _D$, we have $\dot{u}=0$ on $\Ga _D$ and also $\nabla u = \displaystyle \frac{\pa u}{\pa n}n$. Now, from the definition of the shape derivative $u'$ we get that
    
    \noindent
    \begin{equation*}
    	u'=\dot{u}-\frac{\pa u}{\pa n}V\cdot n=-\frac{\pa u} {\pa n}V\cdot n \text{ on }\Ga _D.
    \end{equation*}
    %Again using the identity $\nabla (\nabla u\cdot V)=\nabla ^2 u V+{DV}^T\nabla u$, we get that:
    %\noindent
    On $\Ga _N$
    %\[\frac{\pa u'}{\pa n}=\nabla u\cdot n = \frac{\pa \dot{u}}{\pa n}- \nabla (\nabla u\cdot V)\cdot n \]
    %
    
    \noindent
    \begin{equation*}
    	%\begin{aligned}
    	\frac{\pa u'}{\pa n}
    	%&
    	= \frac{\pa \dot{u}}{\pa n}- \nabla (\nabla u\cdot V) \cdot n
    	=-\big(A'(0)\nabla u +\nabla (\nabla u \cdot V)\big)\cdot n.%\qedhere
    	% &= -\mathrm{div} (V)\frac{\pa u}{\pa n}+DV\nabla u \cdot n
    	%+{DV}^T\nabla u\cdot n- \nabla^2u V\cdot n - {DV}^T \nabla u\cdot n \\
    	% &= DV\nabla u\cdot n- \nabla^2u V\cdot n.
    	%\end{aligned}
    \end{equation*}
    This completes the proof.
%    \begin{eqnarray*}
%    	\frac{\pa u'}{\pa n}
%    	&=& \frac{\pa \dot{u}}{\pa n}- \nabla (\nabla u\cdot V)\cdot n
%    	 =-(A'(0)\nabla u)\cdot n - \nabla^2uV\cdot n - DV^*\nabla u\cdot n\\
%    	&=& -\mathrm{div} (V)\frac{\pa u}{\pa n}+DV\nabla u\cdot n
%    	 +DV(0)^*\nabla u\cdot n- \nabla^2uV\cdot n - DV^*\nabla u\cdot n\\
%    	&=& DV\nabla u\cdot n- \nabla^2uV\cdot n. \qedhere
%    \end{eqnarray*}
    %
    %Showing \eqref{shape:eqn1}:
    %
%\begin{multline*}
%	\int_\Om\Big( \nabla(\nabla u\cdot V)+ (A'(0)\nabla u)\Big)\cdot \nabla \varphi\dx\\
%	=\int_\Om\Big(\nabla^2uV+DV^T\nabla u+\mathrm{div}(V)\nabla u-DV\nabla u-DV^T\nabla u\Big)\cdot \nabla \varphi\dx\\
%	=\int_\Om\Big(\nabla \times (\nabla u\times V)+\De u V\Big)\cdot \nabla\varphi\dx=0-\tau\int_\Om u V\cdot\nabla\varphi\dx=\tau\int_\Om \mathrm{div}(uV)\varphi\dx.
%\end{multline*}
%\tr{Proof yet to finish.}
\end{proof}
%
\par Next, we compute the Eulerian derivative of the first eigenvalue $\tau _1(\Om )$ of~\eqref{eigen1}.
%
\begin{theorem}\label{thm:shape}
	Let $V$ be a vector field given in~\eqref{trans}. If $\tau _1(\Om )$ is the first eigenvalue of~\eqref{eigen1} and $u$ is an eigenfunction corresponding to $\tau _1(\Om )$ with the normalization $\int _\Om u^2 \dx=1$, then the Eulerian derivative of $\tau _1(\Om )$ in the direction of $V$ is given by
	%
	\begin{equation}\label{shape formula}
		d\tau(\Om ;V)=\int _{\Ga _N} \left(\md{\nabla u}^2-\tau _1(\Om ) u^2\right)\, (V\cdot n) \dS - \int _{\Ga _D} \left(\frac{\partial u}{\partial n}\right)^2\, (V\cdot n) \dS.
	\end{equation}
	%
\end{theorem}
%
\begin{proof}
	%From the variational characterization of $\tau _1(\Om )$, we have $\tau _1(\Om ) = \int _{\Om } \md{\nabla u}^2 \dx,$ for an eigenfunction $u$ with $\int _{\Om }u^2\dx =1.$
	Firstly, we recall (from \cite[Theorem 3.3]{Simon80}) that, if a shape functional $J(\Om )$ is given by $J(\Om )=\int _\Om C(u(\Om ))\dx$ under the assumptions that:  the operator $C:W^{1,p}(\Om )\longrightarrow L^1(\Om )$ is differentiable, and both the functions $u(\Om )\in W^{1,p}(\Om )$ and $C(u(\Om ))\in W^{1,1}(\Om )$ have the material derivative in the direction of $V$, then the Eulerian derivative of $J$ in the direction of $V$ exists and is given by %a shape functional of the form $J(\Om )=\int _{\Om }C(u)\dx$, for a nice differential operator $C(\cdot )$, in the direction of the vector field $V$ is given by
	\begin{equation}\label{shape derivative}
	\mathrm{d}J(\Om ;V)=\int _\Om \frac{\pa C}{\pa u}(u')\dx + \int _{\pa \Om }C(u)(V\cdot n)\dS.
	\end{equation}
	Let $u$ be an eigenfunction corresponding to $\tau _1(\Om )$ with the normalization $\int _\Om u^2 \dx=1$. From Proposition~\ref{mat_der}, the material derivatives of $u(\Om )$ and $C(u(\Om ))$ exist, and therefore the Eulerian derivative of the shape functionals $\int _\Om |\nabla u|^2 \dx $ and $\int _\Om u^2 \dx $ exist. %From the variational characterization, we have $\tau _1(\Om )=\int _\Om |\nabla u|^2\dx $ for a corresponding eigenfunction $u(\Om )$ with the normalization $\int _\Om u^2 \dx =1$. 
	By taking shape derivative of $\int _{\Om }u^2\dx =1$ in the direction of $V$ on both sides, and using \eqref{shape derivative} together with the boundary conditions yields
	%
	\begin{equation}\label{shape:l2}
        %2\displaystyle\int_{\Om} u u^{\prime}+\int_{\partial\Om}u^2 \, (V\cdot n) \dS =0 \ \Longrightarrow 
        2 \int _{\Om } u u'\dx +\int _{\Ga _N} u^2 \, (V\cdot n) \dS =0.
    \end{equation}
    %
    Notice that, $\tau _1(\Om )=\int _\Om |\nabla u|^2 \dx $. Thus, again by~\eqref{shape derivative}, we get
    
    \noindent
    \begin{equation*}
    	d\tau _1(\Om ;V)
    	=2 \int _{\Om }\nabla u\cdot \nabla u'\dx
    	+ \int _{\pa \Om}\md{\nabla u}^2\, (V\cdot n) \dS.
    \end{equation*}
    Since $u$ is constant on $\Ga_D$, we have
    $\nabla u =\displaystyle \frac{\pa u}{\pa n}n$
    and
    $\md{\nabla u}= \md{\displaystyle \frac{\partial u}{\partial n}}$
    on $\Ga _D$. Therefore %From \eqref{shape derivative}, we have:
    %
    \begin{equation}\label{shape_der1}
    	d\tau _1(\Om ;V)
    	=2 \int _{\Om}\nabla u\cdot \nabla u'\dx
    	+\int_{\Ga _D} \left(\frac{\pa u}{\pa n}\right)^2\, (V\cdot n) \dS +\int _{\Ga _N}\md{\nabla u}^2\, (V\cdot n) \dS.
  \end{equation}
    %
    By multiplying the equation $-\De u=\tau _1(\Om )u$ with $u'$ and then using the integration by parts we obtain % From the weak formulation of \eqref{eigen}, we have %\[\displaystyle\int_{\Om} \nabla u\cdot \nabla u^{\prime}- \int_{\Ga_D} \frac{\partial u}{\partial n}u^{\prime} \dS = \la\int_{\Om}u u^{\prime}\ \Longrightarrow\displaystyle2\int_{\Om} \nabla u\cdot \nabla u^{\prime} \dS =2\la\int_{\Om}u u^{\prime} -2\int_{\Ga_D} \left(\frac{\partial u}{\partial n}\right)^2 \t\cdot n \dS. \]
    \begin{equation}\label{shape_der2}
    	\int _{\Om } \nabla u\cdot \nabla u'\dx- \int _{\Ga _D} \frac{\pa u}{\pa n} u^{\prime } \dS = \tau _1(\Om ) \int _{\Om }u u'\dx.
    \end{equation}
    By combining~\eqref{shape:l2}-\eqref{shape_der2}, we get:
    %
%    
%    \noindent
%    \begin{equation*}
%    	2\int _{\Om }\nabla u\cdot \nabla u' \dx=-\tau _1(\Om ) \int _{\Ga _N} u^2 \, (V\cdot n) \dS -2\int _{\Ga _D} \left(\frac{\pa u}{\pa n}\right)^2 \, (V\cdot n) \dS.
%    \end{equation*}
%    %
%    Therefore
    
    \noindent
    \begin{equation*}
    	d\tau _1(\Om ;V)= \int _{\Ga _N} \left(\md{\nabla u}^2-\tau _1(\Om ) u^2\right)\, (V\cdot n) \dS - \int _{\Ga _D} \left(\frac{\pa u}{\pa n}\right)^2\, (V\cdot n) \dS. \qedhere
    \end{equation*}
    %
\end{proof}
%
For a similar shape derivative formula for the Dirichlet eigenvalue, we refer to \cite{Anoop18, Zivari08}.
